Speaker Information Can Guide Models to Better Inductive Biases: A Case Study On Predicting Code-Switching

Natural language processing (NLP) models trained on people-generated data can be unreliable because, without any constraints, they can learn from spurious correlations that are not relevant to the task. We hypothesize that enriching models with speaker information in a controlled, educated way can guide them to pick up on relevant inductive biases. For the speaker-driven task of predicting code-switching points in English--Spanish bilingual dialogues, we show that adding sociolinguistically-grounded speaker features as prepended prompts significantly improves accuracy. We find that by adding influential phrases to the input, speaker-informed models learn useful and explainable linguistic information. To our knowledge, we are the first to incorporate speaker characteristics in a neural model for code-switching, and more generally, take a step towards developing transparent, personalized models that use speaker information in a controlled way.

==> tables/test_results_table.tex <==
% \begin{table*}
% \centering
% \begin{tabular}{llcccc}
% \hline \textbf{Model Type} & \textbf{Context} & \textbf{Acc. (\%)}  & \textbf{F1} & \textbf{Recall} & \textbf{Precision}\\ \hline

% \hline
% Majority & - & 76.6 & -- & -- & -- \\ 
% \hline
% List & 1 & 86.630 $\pm$ 1.28 & 0.748 $\pm$ 0.012 & 0.845 $\pm$ 0.032 & 0.673 $\pm$ 0.033 \\
% List & 2 & 86.948 $\pm$ 0.82 &  0.753 $\pm$ 0.010 & 0.848 $\pm$ 0.015 & 0.677 $\pm$ 0.022 \\
% List & 3 & 86.766 $\pm$ 1.0075 & 0.7488 $\pm$ 0.011 &  0.8418 $\pm$ 0.021 & 0.676 $\pm$ 0.0286 \\
% List & 5 & 86.808 $\pm$ 1.00  & 0.752 $\pm$ 0.013 &  0.8516 $\pm$ 0.0184 & 0.6734 $\pm$ 0.0262 \\
% Partner  & 1  & 86.7058 $\pm$ 0.96 & 0.7419 $\pm$ 0.0086 &  0.8157 $\pm$ 0.024 & 0.6819 $\pm$ 0.028 \\
% Partner  & 2 &  87.0110 $\pm$ 1.068 & 0.7510 $\pm$ 0.012 &  0.8365 $\pm$ 0.038 &  0.6840 $\pm$ 0.034 \\
% Partner & 3  & 87.1657 $\pm$ 0.8367 &  0.7528 $\pm$ 0.011 & 0.8347 $\pm$ 0.021 & 0.6864 $\pm$ 0.024 \\
% Partner  & 5   &  87.0605 $\pm$ 0.68 & 0.7511 $\pm$ 0.0074 & 0.8340 $\pm$ 0.014 & 0.6837 $\pm$ 0.019\\
% Sentence & 1 & 86.1933 $\pm$ 0.6615 & 0.7389 $\pm$ 0.011 & 0.8352 $\pm$ 0.027 & 0.6632 $\pm$ 0.017\\
% Sentence  & 2 &  86.8392 $\pm$ 1.20 & 0.7499 $\pm$ 0.013 &  0.8414 $\pm$ 0.022 &  0.6777 $\pm$ 0.031\\
% Sentence  & 3  & 86.9483 $\pm$ 1.20 & 0.7523 $\pm$ 0.013 & 0.8453 $\pm$ 0.021 & 0.6793 $\pm$ 0.033\\
% Sentence  & 5 &  87.0080 $\pm$ 0.7643 & 0.7528 $\pm$ 0.0092 & 0.8450 $\pm$ 0.022 & 0.6796 $\pm$ 0.021 \\
% XLM-R Base  & 1 & 85.6333 $\pm$ 0.9170 & 0.7391 $\pm$ 0.0081 & 0.8689 $\pm$ 0.022 & 0.6440 $\pm$ 0.022\\
% XLM-R Base  & 2 & 85.4988 $\pm$ 0.7637 & 0.7396 $\pm$ 0.0067 & 0.8796 $\pm$ 0.020 & 0.6388 $\pm$ 0.020\\
% XLM-R Base  & 3 & 85.6808 $\pm$ 0.8393 & 0.7436 $\pm$ 0.0088 & 0.8866 $\pm$ 0.013 & 0.6407 $\pm$ 0.018\\
% XLM-R Base  & 5 & 86.0871 $\pm$ 1.1974 & 0.7494 $\pm$ 0.013 & 0.8876 $\pm$ 0.020 & 0.6495 $\pm$ 0.027\\
% \hline
% \end{tabular}
% \caption{\label{tab:val-results} Performance of all models on the test set (23.4\% code-switched). }
% \end{table*}


\begin{table*}[h!]
\centering
\scalebox{0.8}{
\begin{tabular}{llcccc}
\hline \textbf{Model Type} & \textbf{Context} & \textbf{Acc. (\%)}  & \textbf{F1} & \textbf{Recall} & \textbf{Precision}\\ \hline

\hline
Majority & - & 74.8 & -- & -- & -- \\ 
\hline
List & 1 & 78.9 $\pm$ 1.247 & 61.4 & 66.7 & 57.2 \\
List & 2 & 79.7 $\pm$ 1.063 &  63.0 & 68.5 & 58.4 \\
List & 3 & 80.0 $\pm$ 0.769 & 64.0 & 70.4 & 58.8 \\
List & 5 & 80.2 $\pm$ 0.919  & 64.3 & 70.9 & 59.0 \\
Partner  & 1  & 78.5 $\pm$ 1.966 & 59.8 & 63.5 & 57.0 \\
Partner  & 2 &  79.4 $\pm$ 1.120 & 62.4 & 67.8 & 58.1 \\
Partner  & 3 &  80.0 $\pm$ 0.927 & 63.5 & 69.0 & 58.9 \\
Partner & 5  & 79.5 $\pm$ 1.268 &  62.9 & 69.2 & 58.1 \\
Sentence  & 1   &  79.0 $\pm$ 1.260 & 60.9 & 65.9 & 57.5\\
Sentence & 2 & 79.6 $\pm$ 1.095 & 63.4 & 70.4 & 57.9\\

Sentence  & 3  & 80.0 $\pm$ 1.021 & 63.4 & 69.4 & 58.6\\
Sentence  & 5 &  79.4 $\pm$ 1.602 & 64.4 & 74.2 & 57.3 \\
XLMR  & 1 & 69.5 $\pm$ 2.755 & 56.5 & 78.7 & 44.3\\
XLMR  & 2 & 71.8 $\pm$ 2.231 & 58.7 & 79.7 & 46.7\\
XLMR  & 3 & 72.4 $\pm$ 2.312 & 59.8 & 81.3 & 47.4\\
XLMR`  & 5 & 74.2 $\pm$ 2.394 & 61.2 & 80.9 & 49.5\\
\hline
\end{tabular}
}
\caption{\label{tab:val-results} Performance of all models on the test set (25.2\% code-switched). }
\end{table*}


==> tables/val_results_table.tex <==
% \begin{table*}
% \centering
% \begin{tabular}{llcccc}
% \hline \textbf{Model Type} & \textbf{Context} & \textbf{Acc. (\%)}  & \textbf{F1} & \textbf{Recall} & \textbf{Precision}\\ \hline

% \hline
% Majority & - & 76.2 & -- & -- & -- \\ 
% \hline
% List & 1 & 83.917 $\pm$ 1.45 & 0.719 $\pm$ 0.014 & 0.864 $\pm$ 0.021 & 0.617 $\pm$ 0.028 \\
% List & 2 & 84.673 $\pm$ 1.13 &  0.7263 $\pm$ 0.0108 & 0.8541 $\pm$ 0.0194 & 0.6328 $\pm$ 0.0253 \\
% List & 3 & 84.9493 $\pm$ 1.2061 & 0.7290 $\pm$ 0.0122 &  0.8499 $\pm$ 0.0177 & 0.6393 $\pm$ 0.0278 \\
% List & 5 & 84.9873 $\pm$ 0.9465  & 0.7303 $\pm$ 0.0109 &  0.8540 $\pm$ 0.0147 & 0.6384 $\pm$ 0.0214 \\
% Partner  & 1  & 84.1763 $\pm$ 1.5531 & 0.7191 $\pm$ 0.0142 &  0.8493 $\pm$ 0.0235 & 0.6250 $\pm$ 0.0319 \\
% Partner  & 2 &  84.6381 $\pm$ 1.5288 & 0.7273 $\pm$ 0.0143 &  0.8591 $\pm$ 0.0258 &  0.6324 $\pm$ 0.0338 \\
% Partner & 3  & 84.7311 $\pm$ 1.1342 &  0.7276 $\pm$ 0.0116 & 0.8562 $\pm$ 0.0191 & 0.6335 $\pm$ 0.0264 \\
% Partner  & 5   &  84.7916 $\pm$ 0.5420 & 0.7287 $\pm$ 0.0051 & 0.8589 $\pm$ 0.0124 & 0.6330 $\pm$ 0.0122\\
% Sentence & 1 & 83.8130 $\pm$ 0.7906 & 0.7141 $\pm$ 0.0086 & 0.8499 $\pm$ 0.0160 & 0.6161 $\pm$ 0.0161\\
% Sentence  & 2 &  85.0493 $\pm$ 1.0879 & 0.7288 $\pm$ 0.0106 &  0.8437 $\pm$ 0.0180 &  0.6423 $\pm$ 0.0242\\
% Sentence  & 3  & 85.1929 $\pm$ 1.1840 & 0.7308 $\pm$ 0.0117 & 0.8438 $\pm$ 0.0188 & 0.6457 $\pm$ 0.0286\\
% Sentence  & 5 &  85.1070 $\pm$ 1.0274 & 0.7315 $\pm$ 0.0115 & 0.8521 $\pm$ 0.0124 & 0.6414 $\pm$ 0.0227 \\
% XLM-R Base  & 1 & 82.9414 $\pm$ 1.2593 & 0.7096 $\pm$ 0.0109 & 0.8751 $\pm$ 0.0198 & 0.5976 $\pm$ 0.0235\\
% XLM-R Base  & 2 & 83.1484 $\pm$ 0.9166 & 0.7141 $\pm$ 0.0073 & 0.8844 $\pm$ 0.0189 & 0.5994 $\pm$ 0.0192\\
% XLM-R Base  & 3 & 83.3906 $\pm$ 1.0227 & 0.7186 $\pm$ 0.0097 & 0.8912 $\pm$ 0.0134 & 0.6025 $\pm$ 0.0187\\
% XLM-R Base  & 5 & 83.6187 $\pm$ 1.1898 & 0.7209 $\pm$ 0.0100 & 0.8884 $\pm$ 0.0212 & 0.6075 $\pm$ 0.0236\\
% \hline
% \end{tabular}
% \caption{\label{tab:val-results} Performance of all models on the validation set (23.8\% code-switched). }
% \end{table*}
\begin{table*}[h!]
\centering
\scalebox{0.6}{
\begin{tabular}{llcccc}
\hline \textbf{Model Type} & \textbf{Context} & \textbf{Acc. (\%)}  & \textbf{F1} & \textbf{Recall} & \textbf{Precision}\\ \hline

\hline
Majority & - & 75.0 & -- & -- & -- \\ 
\hline
List & 1 & 75.9 $\pm$ 1.390 & 60.1 & 72.3 & 51.5 \\
List & 2 & 77.4 $\pm$ 0.932 &  60.9  &  70.4 & 53.8 \\
List & 3 & 78.3 $\pm$ 1.191 & 62.0 & 71.0 & 55.3\\
List & 5 & 78.9 $\pm$ 1.418 & 63.1 & 72.1 & 56.4 \\
Partner  & 1  & 77.4 $\pm$ 2.301 & 61.1 & 70.6 & 54.1\\
Partner  & 2 &  78.3 $\pm$ 0.966 & 61.8 & 70.4 & 55.2 \\
Partner & 3  & 78.7 $\pm$ 0.982 &  62.6 & 71.2 & 55.9 \\
Partner  & 5   &  78.8 $\pm$ 1.228 & 62.9 & 71.7 & 56.2\\
Sentence & 1 & 77.5 $\pm$ 1.667 & 60.5 & 68.9 & 54.2\\
Sentence  & 2 &  77.9 $\pm$ 1.210 & 61.6 & 71.0 & 54.6\\
Sentence  & 3  & 78.2 $\pm$ 1.255 & 62.1 & 69.5 & 56.3\\
Sentence  & 5 &  78.2 $\pm$ 1.863 & 63.2 & 74.5 & 55.1 \\
XLMR  & 1 & 66.4 $\pm$ 2.836 & 54.0 & 78.9 & 41.3\\
XLMR  & 2 & 70.3 $\pm$ 3.269 & 57.2& 79.0 & 45.2\\
XLMR  & 3 & 71.4 $\pm$ 1.916 & 58.2 & 79.6 & 46.0\\
XLMR  & 5 & 73.1 $\pm$ 2.739 & 59.8 & 79.9 & 48.0\\
\hline
\end{tabular}
}
\caption{\label{tab:val-results} Performance of all models on the validation set (25.0\% code-switched). }
\end{table*}
